Early Planet Formation in Embedded Disks (eDisk). II. Limited Dust Settling and Prominent Snow Surfaces in the Edge-on Class I Disk IRAS 04302+2247

While dust disks around optically visible, Class II protostars are found to be vertically thin, when and how dust settles to the midplane are unclear. As part of the Atacama Large Millimeter/submillimeter Array (ALMA) large program, Early Planet Formation in Embedded Disks, we analyze the edge-on, embedded, Class I protostar IRAS 04302+2247, also nicknamed the ``Butterfly Star." With a resolution of 0.05" (8~au), the 1.3 mm continuum shows an asymmetry along the minor axis which is evidence of an optically thick and geometrically thick disk viewed nearly edge-on. There is no evidence of rings and gaps, which could be due to the lack of radial substructure or the highly inclined and optically thick view. With 0.1" (16~au) resolution, we resolve the 2D snow surfaces, i.e., the boundary region between freeze-out and sublimation, for $^{12}$CO $J$=2--1, $^{13}$CO $J$=2--1, C$^{18}$O $J$=2--1, $H_{2}$CO $J$=$3_{0,3}$--$2_{0,2}$, and SO $J$=$6_{5}$--$5_{4}$, and constrain the CO midplane snow line to $\sim 130$ au. We find Keplerian rotation around a protostar of $1.6 \pm 0.4 M_{\odot}$ using C$^{18}$O. Through forward ray-tracing using RADMC-3D, we find that the dust scale height is $\sim 6$ au at a radius of 100~au from the central star and is comparable to the gas pressure scale height. The results suggest that the dust of this Class~I source has yet to vertically settle significantly.

==> deleted_content.tex <==
%%% section on large scale emission of 12co and 13co
\red{need to add a transition. For young edge-on disks, the large scale emission can provide formation context to the dis formation process}
The largest scale emissions for $^{13}$CO and $^{12}$CO are illustrated by the integrated intensity images in Fig.~\ref{fig:moments_redblue}. For $^{12}$CO, the blue color maps are produced within the velocity range of -6.03 to 3.50 km s$^{-1}$, while the red color maps are produced from 7.30 to 16.83 km s$^{-1}$. For $^{13}$CO, the blue color maps are produced within the velocity range of 0.01 to 5.69 km s$^{-1}$, while the red color maps are produced from 6.36 to 12.04 km s$^{-1}$. Both lines used robust=2 to capture the large scale emission. However, given that $^{12}$CO appears less extended than $^{13}$CO, it is likely that $^{12}$CO remains resolved out. \red{take out this figure, since there's no point to be made here}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{moments_multi_SBLB_redblue.pbcor.pdf}
    \caption{
        Integrated intensity images for $^{12}$CO (left) and $^{13}$CO (right) using only red-shifted or blue-shifted channels. The 5$\sigma$ level of the continuum is outlined in grey. The white line segment to the lower right is 500~au length scale. \red{put velocity range here}. \red{grey is hard to see}
    }
    \label{fig:moments_redblue}
\end{figure*}




%%% section on complex structures of 12CO
\subsection{Complex Structures of $^{12}$CO} \label{sec:12co_complex}

Similar to $^{13}$CO, $^{12}$CO traces several complicated structures that do not appear to follow the typical Keplerian rotation of a disk. Fig.~\ref{fig:channel_12co_features} shows selected channel maps to present the complexities. This section aims to identify these structures from the following guidelines: (1) the emission is above 3$\sigma$, (2) the emission is clearly not part of the Keplerian rotating disk, and (3) the emission is seen across multiple channels. We named the features as Feature 1 to 4 (F1-4)without assuming the nature of the emission. We caution that although some features may appear connected across channels, it could be an overlap of spatially distinct features. 


Starting from the most obvious, Feature 1 is an extended material (with size $\sim 3\arcsec$) that lies along the blue-end of the jet axis (in the east) at the blue-shifted channels (from $\sim -1$ to $3.5$ km s$^{-1}$). The feature is more blue-shifted further away from the disk. In addition, the northern half (bisected by the jet axis) appears more blue-shifted than the southern half. Given that the blob is along the jet axis, it is likely a blue-shifted rotating outflow. The rotation direction is consistent with the disk. 

Feature 2 is a long thin tail in the northeast at low blue-shifted channels (from $2.4$ to $3.5$ km s$^{-1}$). The shape is marked by a parabola $y = 0.15 x^{2} + 1.5$. The northern most point is most blue-shifted, whereas the southern most point appears to connect the disk surface at $\sim 2 \arcsec$ (320 au) above the midplane. Given that the furthest point is also the most blue-shifted, the tail is likely part of an outflow phenomena \red{reference}. 

Feature 3 appears as a long arc in the west side of the disk. The arc appears parallel to the disk major axis (at $\sim 2\arcsec$ from the disk center) seen in $7.31-7.95$ km s$^{-1}$ channels and then connects the disk surface in the red-shifted channels ($7.31 - 9.22$ km s$^{-1}$). Without assuming the origin of the shape, Feature 3 is marked by a rotated parabola given by the following procedure. The parabola $x = 2 y^{2}$ is rotated by $15^{\circ}$ east-of-north, then translated by ($-2.2\arcsec$, $-1.8\arcsec$). Given that the point of the arc that is closest to the disk appears in the most red-shifted channel and that the outer part of the arc is closer to the system velocity, it is better explained by infall motion. The projected parabolic shape can potentially be explained by a spiral that is not confined to the midplane, but instead elevated depending on the location. 

Feature 4 is a straight spike-like feature in the west that appears to protrude from the disk surface. The feature is most prominent and extended in the red-shifted channels ($\sim 7.31 - 8.58$ km s$^{-1}$), but the feature appears in blue-shifted channels near the base of the spike, too. The nature of Feature 4 is unclear. Given that, in the red-shifted half, the emission is concentrated closer to the disk surface at higher velocities, it is more consistent with infall motion in which case the material falls in front of the plane of sky. However, the scenario cannot explain the blue-shifted part of the feature. \red{John Tobin: I think an outflow driven by a disk wind can have spatial overlap in the red- and blue-shifted emission.}


\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{channel_12co_features.pdf}
    \caption{
        \red{need to add a colorbar} Selected channel images of $^{12}$CO with robust=2.0. The contours outline the $5\sigma$ level. The central channels from $3.6 \sim 7$~km s$^{-1}$ were taken out, since those were resolved out and largely featureless. We show the snow surface in white. The features are labeled F1 to F4 in the first channel (see Section~\ref{sec:12co_complex} for details). 
    }
    \label{fig:channel_12co_features}
\end{figure*}



